Two- and Three-Particle Jet-Like Correlations

We present results of 2-particle jet-like correlations, with high pT h+- triggers and identified pi+-, p, and pbar triggers in d+Au and Au+Au collisions and 3-particle jet-like azimuthal correlations in pp, d+Au, and Au+Au collisions at sqrt(s)=200 GeV. These results use data from the STAR TPC during RHIC runs II, III, and IV. Modifications in 2-particle correlations are observed in Au+Au collisions. These modifications are not seen in $pp$ or d+Au collisions. This demonstrates that the modifications are due to final state nuclear effects. High pT protons, anti-protons and charged pions are identified by the relativistic rise of dE/dx in the STAR TPC. Correlations of charged hadrons with high pT p, pbar, and pi+- show no discernible difference. The results post challenges to recombination and coalescence models which are otherwise very successful in explaining the large baryon/meson ratio and the splitting of the elliptic flow at intermediate pT. In central Au+Au collisions, the away-side 2-particle correlation is significantly broadened and even double humped in selective kinematic ranges. Three-particle correlations were employed to identify the underlying physics mechanism(s). Results in pp, d+Au and peripheral Au+Au collisions show dijet structure with away-side kT broadening. Results in mid-central and central Au+Au collisions are consistent with a near-side jet and on the away-side a combination of conical emission and large angle gluon radiation and deflected jets. The associated pT independent emission angle suggests Mach-cone shock waves being the underlying physics mechanism for the conical emission. The emission angle is measured to be 1.39+-0.01 (stat.)+-0.04(sys.) in ZDC triggered 0-12% Au+Au data.

==> tables.tex <==
%
%  tables.tex   2004.10.14  13:38:03   Mark Senn <mark@purdue.edu>
%
%  Demonstrate how to do tables.
%

\chapter{Tables}

\newlength{\ta}
\newlength{\tb}
\newlength{\tc}

\settowidth{\ta}{\vbox{\hbox{Money}\hbox{Market}}}
\settowidth{\tb}{\vbox{\hbox{Stocks}\hbox{and}\hbox{Bonds}}}
\settowidth{\tc}{\vbox{\hbox{Money}\hbox{Market}\hbox{and}\hbox{Stocks}}}

\makeatletter
%\def\fnum@table{\tablename~\thetable.~}
\makeatother

%{\renewcommand{\baselinestretch}{1}
%  \begin{table}
%    \caption{%
%      \hfil Allocation of the IRA and Keogh Wealth\hfil\break
%      \mbox{}\hfil for Investors With or Without Brokerage Accounts\hfil
%    }
%    \label{tab:ira}
%    \begin{center}
%      \begin{tabular}%
%        {%
%          |%
%          c%
%          |%
%          >{\centering\hspace{0pt}}m{\the\ta}%  Money Market
%          |%
%          c%                                    Stocks 
%          |%
%          c%                                    Bonds
%          |%
%          c%                                    Diversified
%          |%
%          >{\centering\hspace{0pt}}m{\the\tb}%  Stocks and Bonds
%          |%
%          >{\centering\hspace{0pt}}m{\the\tc}%  Money Market and Stocks
%          |%
%          c%                                    Others
%          |%
%        }
%        \hline
%        IMP&
%          Money Market&
%          Stocks&
%          Bonds&
%          Diversified&
%          Stocks and Bonds&
%          Money Market and Stocks&
%          Others\tabularnewline
%        \hline
%        1& 14.19\%& 57.71\%& 12.21\%& 4.50\%& 7.36\%& 3.04\%& 0.99\%\tabularnewline \hline
%        2& 14.08\%& 58.18\%& 12.32\%& 4.44\%& 7.30\%& 2.80\%& 0.88\%\tabularnewline \hline
%        3 &14.26\%& 58.09\%& 12.27\%& 4.50\%& 7.19\%& 2.75\%& 0.94\%\tabularnewline \hline
%        4 &13.94\%& 58.11\%& 12.14\%& 4.78\%& 7.35\%& 2.68\%& 0.99\%\tabularnewline \hline
%        5 &13.92\%& 58.13\%& 11.93\%& 4.56\%& 7.60\%& 2.98\%& 0.88\%\tabularnewline \hline
%      \end{tabular}
%    \end{center}
%    This table presents the allocations of the wealth in the IRA
%    and Keogh accounts in various asset classes.
%    Results from each set of imputed data are presented here.
%    The first column lists the number of the imputations,
%    and rest of the columns lists various allocations.
%    Entrees under each asset class show the percentage of investors
%    who have most of their IRA
%    and Keogh wealth invested in that particular asset class.
%    The asset class Diversified
%    includes stocks,
%    bonds,
%    and money market investments.
%    The asset class Others
%    include investments in various life insurance products,
%    annuities,
%    real estate, etc.
%    \medskip
%    \footnotesize SOURCE: Survey of Consumer Finances,
%    2001,
%    Federal Reserve Board,
%    USA.\par
%  \end{table}
%}
%


\begin{table}
This is the table that contains only text.
Let's cite Lamport:1994 here: \cite{Lamport:1994}.
\caption{%
  This is the caption.
  Let's cite Lamport:1994 here: \cite{Lamport:1994}%
}
\end{table}

\begin{table}
  \hbox to \textwidth{\hfill\vbox{\halign{
    \strut #&            % 0. \strut
    #\hfil\qquad&        % 1. left
    \hfil #\hfil\qquad&  % 2. center
    \hfil #\cr           % 3. right
    %
    & apple& banana& cherry\cite{Lamport:1994}\cr
    & aardvark& boa constrictor& coyote\cr
  }}\hfill}
  \caption[2.1short caption for table of contents]{This is a really long and boring caption.  It goes
on and on as if it thinks what it says is important.  Here is
some more of it.  And here is one final sentence.\cite{Lamport:1994}}
\end{table}

  % This is loosely based on page 106 of _A Guide to LaTeX_, third edition,
  % by Helmut Kopka and Patrick W. Daly.
%\begin{longtable}{|l|l|}
%  \caption{2.2 ``State'' Abbreviations}\\
%  \hline
%  ``State''& Abbreviation\\
%  \hline \endfirsthead
%  \caption[]{\emph{continued}}\\
%  \hline
%  ``State''& Abbreviation\\
%  \hline \endhead
%  \hline
%  \multicolumn{2}{r}{\emph{continued on next page}}
%  \endfoot
%  \hline\endlastfoot
%  Alabama& AL\\
%  Alaska& AK\\
%  American Samoa& AS\\
%  Arizona& AZ\\
%  Arkansas& AR\\
%  Armed Forces Europe& AE\\
%  Armed Forces Pacific& AP\\
%  Armed Forces the Americas& AA\\
%  California& CA\\
%  Colorado& CO\\
%  Connecticut& CT\\
%  Delaware& DE\\
%  District of Columbia& DC\\
%  Federated States of Micronesia& FM\\
%  Florida& FL\\
%  Georgia& GA\\
%  Guam& GU\\
%  Hawaii& HI\\
%  Idaho& ID\\
%  Illinois& IL\\
%  Indiana& IN\\
%  Iowa& IA\\
%  Kansas& KS\\
%  Kentucky& KY\\
%  Louisiana& LA\\
%  Maine& ME\\
%  Marshall Islands& MH\\
%  Maryland& MD\\
%  Massachusetts& MA\\
%  Michigan& MI\\
%  Mississippi& MS\\
%  Missouri& MO\\
%  Montana& MT\\
%  N Minnesota
%  Nebraska& NE\\
%  Nevada& NV\\
%  New Hampshire& NH\\
%  New Jersey& NJ\\
%  New Mexico& NM\\
%  New York& NY\\
%  North Carolina& NC\\
%  North Dakota& ND\\
%  Northern Mariana Islands& MP\\
%  Ohio& OH\\
%  Oklahoma& OK\\
%  Oregon& OR\\
%  Pennsylvania& PA\\
%  Puerto Rico& PR\\
%  Rhode Island& RI\\
%  South Carolina& SC\\
%  South Dakota& SD\\
%  Tennessee& TN\\
%  Texas& TX\\
%  Utah& UT\\
%  Vermont& VT\\
%  Virgin Islands, U.S.& VI\\
%  Virginia& VA\\
%  Washington& WA\\
%  West Virginia& WV\\
%  Wisconsin& WI\\
%  Wyoming& WY\\
%\end{longtable}

\newcommand{\cbackslash}{\char'134}
\newcommand{\copencurly}{\char'173}
\newcommand{\cclosecurly}{\char'175}

\newlength{\twidth}
\newlength{\theight}

\setlength{\twidth}{\textwidth}
\setlength{\theight}{\textheight}

\begin{sidewaystable}
    % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}
  \setlength{\textheight}{\twidth}
  \caption{2.3 sidewaystable mode {\tt\cbackslash begin\copencurly table\cclosecurly\/}\ldots{\tt\cbackslash end\copencurly table\cclosecurly\/} table}
  \hbox to \textwidth{\hfill
    \begin{tabular}{lcr}
      apple& banana& cherry\\
      aardvark& boa constrictor& coyote\\
    \end{tabular}
  \hfill}
\end{sidewaystable}

\begin{sidewaystable}
    % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}
  \setlength{\textheight}{\twidth}
  \caption{2.4 sidewaystable mode {\tt\cbackslash halign\copencurly ...\cclosecurly\/} table}
  \hbox to \textwidth{\hfill\vbox{\halign{
    \strut #&            % 0. \strut
    #\hfil\qquad&        % 1. left
    \hfil #\hfil\qquad&  % 2. center
    \hfil #\cr           % 3. right
    %
    & apple& banana& cherry\cr
    & aardvark& boa constrictor& coyote\cr
  }}\hfill}
\end{sidewaystable}

\begin{table}
  \begin{tabular}{lcr}
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
  \end{tabular}
  \caption{2.5 left hand table}
\end{table}

\begin{table}
  \begin{tabular}{lcr}
    apple& banana& cherry\\
    aardvark& boa constrictor& coyote\\
  \end{tabular}
  \caption{2.6 left hand table}
\end{table}

This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.

\begin{sidewaystable}
    % The following two lines compensate for what I think is a bug.
  \setlength{\textwidth}{\theight}
  \setlength{\textheight}{\twidth}
  \caption{2.7 sidewaystable mode {\tt\cbackslash begin\copencurly table\cclosecurly\/}\ldots{\tt\cbackslash end\copencurly table\cclosecurly\/} table}
  \hbox to \textwidth{\hfill
    \begin{tabular}{lcr}
      apple& banana& cherry\\
      aardvark& boa constrictor& coyote\\
    \end{tabular}
  \hfill}
\end{sidewaystable}

This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.
This is a sentence.  This is a sentence.  This is a setence.

%\newlength{\ta}
%\settowidth{\ta}{\vbox{\hbox{Money}\hbox{Market}}}
%\newlength{\tb}
%\settowidth{\tb}{\vbox{\hbox{Stocks}\hbox{and}\hbox{Bonds}}}
%\newlength{\tc}
%\settowidth{\tc}{\vbox{\hbox{Money}\hbox{Market}\hbox{and}\hbox{Stocks}}}
%
%  {\renewcommand{\baselinestretch}{1}
%\begin{table}
%  \caption{\hfil Allocation of the IRA and Keogh Wealth\hfil\break\mbox{}\hfil for Investors With or Without Brokerage Accounts\hfil}
%  \label{tab:ira}
%  \begin{center}
%    \begin{tabular}%
%      {%
%        |%
%        c%
%        |%
%        >{\centering\hspace{0pt}}m{\the\ta}%  Money Market
%        |%
%        c%                                    Stocks 
%        |%
%        c%                                    Bonds
%        |%
%        c%                                    Diversified
%        |%
%        >{\centering\hspace{0pt}}m{\the\tb}%  Stocks and Bonds
%        |%
%        >{\centering\hspace{0pt}}m{\the\tc}%  Money Market and Stocks
%        |%
%        c%                                    Others
%        |%
%      }
%      \hline
%      IMP&
%        Money Market&
%        Stocks&
%        Bonds&
%        Diversified&
%        Stocks and Bonds&
%        Money Market and Stocks&
%        Others\tabularnewline
%      \hline
%      1& 14.19\%& 57.71\%& 12.21\%& 4.50\%& 7.36\%& 3.04\%& 0.99\%\tabularnewline \hline
%      2& 14.08\%& 58.18\%& 12.32\%& 4.44\%& 7.30\%& 2.80\%& 0.88\%\tabularnewline \hline
%      3 &14.26\%& 58.09\%& 12.27\%& 4.50\%& 7.19\%& 2.75\%& 0.94\%\tabularnewline \hline
%      4 &13.94\%& 58.11\%& 12.14\%& 4.78\%& 7.35\%& 2.68\%& 0.99\%\tabularnewline \hline
%      5 &13.92\%& 58.13\%& 11.93\%& 4.56\%& 7.60\%& 2.98\%& 0.88\%\tabularnewline \hline
%    \end{tabular}
%  \end{center}
%  This table presents the allocations of the wealth in the IRA
%  and Keogh accounts in various asset classes.
%  Results from each set of imputed data are presented here.
%  The first column lists the number of the imputations,
%  and rest of the columns lists various allocations.
%  Entrees under each asset class show the percentage of investors
%  who have most of their IRA
%  and Keogh wealth invested in that particular asset class.
%  The asset class Diversified
%  includes stocks,
%  bonds,
%  and money market investments.
%  The asset class Others
%  include investments in various life insurance products,
%  annuities,
%  real estate, etc.
%  \medskip
%  \footnotesize SOURCE: Survey of Consumer Finances,
%  2001,
%  Federal Reserve Board,
%  USA.\par
%\end{table}
%  }
%

